Photo-astrometric distances, extinctions, and astrophysical parameters for Gaia EDR3 stars brighter than G=18.5

We present a catalogue of 362 million stellar parameters, distances, and extinctions derived from Gaia's early third data release (EDR3) cross-matched with the photometric catalogues of Pan-STARRS1, SkyMapper, 2MASS, and AllWISE. The higher precision of the Gaia EDR3 data, combined with the broad wavelength coverage of the additional photometric surveys and the new stellar-density priors of the {\tt StarHorse} code allow us to substantially improve the accuracy and precision over previous photo-astrometric stellar-parameter estimates. At magnitude $G=14\, (17)$, our typical precisions amount to 3% (15%) in distance, 0.13 mag (0.15 mag) in $V$-band extinction, and 140 K (180 K) in effective temperature. Our results are validated by comparisons with open clusters, as well as with asteroseismic and spectroscopic measurements, indicating systematic errors smaller than the nominal uncertainties for the vast majority of objects. We also provide distance- and extinction-corrected colour-magnitude diagrams, extinction maps, and extensive stellar density maps that reveal detailed substructures in the Milky Way and beyond. The new density maps now probe a much greater volume, extending to regions beyond the Galactic bar and to Local Group galaxies, with a larger total number density. We publish our results through an ADQL query interface ({\tt gaia.aip.de}) as well as via tables containing approximations of the full posterior distributions. Our multi-wavelength approach and the deep magnitude limit make our results useful also beyond the next Gaia release, DR3.

==> im/topcat/stilts <==


# Bailer-Jones+2021

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20  auxmin=-0.3 auxmax=0.3 \
   auxvisible=true auxlabel='dist50/r_{med,\ photogeo} - 1' \
   title='Comparison\ to\ Bailer\mbox{-}Jones+2021\quad (photo\mbox{-}geometric\ distances)' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight='dist50/(r_med_photogeo/1000.) - 1' \
      combine=median  \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_bj2021_skydiff.png

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20  auxmin=-0.3 auxmax=0.3 \
   auxvisible=true auxlabel='dist50/r_{med,\ geo} - 1' \
   title='Comparison\ to\ Bailer\mbox{-}Jones+2021\quad (geometric\ distances)' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight='dist50/(r_med_geo/1000.) - 1' \
      combine=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_bj2021_skydiff2.png
  
topcat -stilts plot2plane \
   xpix=467 ypix=474 \
   xlabel='X_{Gal}\quad [kpc]' \
    ylabel='Y_{Gal}\quad [kpc]' \
    texttype=latex fontsize=21 \
   xmin=-24 xmax=12 ymin=-18 ymax=18 \
   title='Bailer\mbox{-}Jones+2021\ photo\mbox{-}geometric\  distances' \
    legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits x=X_bj21 y=Y_bj21 \
   layer_1=Mark \
      shading_1=density color_1=blue \
       densemap_1=cubehelix \
   layer_2=Contour \
      color_2=white nlevel_2=8 \
       scaling_2=log zero_2=0.7 \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/bj2021_xymap.png
  
topcat -stilts plot2plane \
   xpix=467 ypix=474 \
   xlabel='X_{Gal}\quad [kpc]' \
    ylabel='Y_{Gal}\quad [kpc]' \
    texttype=latex fontsize=21 \
   xmin=-24 xmax=12 ymin=-18 ymax=18 \
   title='StarHorse2021\ (This\ work)' \
    legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits x=XGal y=YGal \
   layer_1=Mark \
      shading_1=density color_1=blue \
       densemap_1=cubehelix \
   layer_2=Contour \
      color_2=white nlevel_2=8 \
       scaling_2=log zero_2=0.7 \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_xymap.png
  
# Bai+2019

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-500 auxmax=500 \
   auxvisible=true auxlabel='teff50 - Teff_{Bai2019}\qquad [K]' \
   title='Comparison\ to\ Bai+2019\quad (T_{\rm eff}\ from\ random\mbox{-}forest\ regression)' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight=teff50-Teff_Bai2019a \
      level=-3 combine=median  \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_bai2019_skydiff.png
  
topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-.5 auxmax=.5 \
   auxvisible=true auxlabel='E(BP-RP)_{SH2019} - E(BP-RP)_{Bai2020}\qquad [mag]' \
   title='Comparison\ to\ Bai+2020\quad (E(BP-RP)\ from\ random\mbox{-}forest\ regression)' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight=phot_bp_mean_mag-phot_rp_mean_mag-BPRP0-e_bp_rp_Bai2019b \
      level=-3 combine=median  \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_bai2020_skydiff_av.png
  
# Andrae+2018

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-500 auxmax=500 \
   auxvisible=true auxlabel='teff50 - Teff_{Andrae+2018}\qquad [K]' \
   title='Comparison\ to\ Andrae+2018\quad (T_{\rm eff}\ from\ {\it Gaia}\ DR2\ {\it Apsis})' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight=teff50-teff_val \
      level=-3 combine=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_andrae2018_skydiff.png
  
topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-.5 auxmax=.5 \
   auxvisible=true auxlabel='AG50 - A_{G_{Andrae+2018}}\qquad [mag]' \
   title='Comparison\ to\ Andrae+2018\quad (A_G\ from\ {\it Gaia}\ DR2\ {\it Apsis})' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight='0.89*av50-a_g_val' \
      level=-3 combine=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_andrae2018_skydiff_av.png
  
# SH2019

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-0.5 auxmax=0.5 \
   auxvisible=true auxlabel='logg50 - logg50_{SH2019}\qquad [dex]' \
   title='Comparison\ to\ Anders+2019\quad (\log g\ from\ {\it Gaia}\ DR2\ {\tt StarHorse})' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight=logg50-logg50_sh2019 \
      combine=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sh2019_skydiff_logg.png
  
topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-500 auxmax=500 \
   auxvisible=true auxlabel='teff50 - teff50_{SH2019}\qquad [dex]' \
   title='Comparison\ to\ Anders+2019\quad (T_{\rm eff}\ from\ {\it Gaia}\ DR2\ {\tt StarHorse})' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight=teff50-teff50_sh2019 \
      combine=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sh2019_skydiff_teff.png
  
topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-0.5 auxmax=0.5 \
   auxvisible=true auxlabel='dist50 - dist50_{SH2019}\qquad [dex]' \
   title='Comparison\ to\ Anders+2019\quad (distances\ from\ {\it Gaia}\ DR2\ {\tt StarHorse})' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight=dist50/dist50_sh2019-1 \
      combine=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sh2019_skydiff_dist.png
  
 topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-0.5 auxmax=0.5 \
   auxvisible=true auxlabel='AV50 - AV50_{SH2019}\qquad [mag]' \
   title='Comparison\ to\ Anders+2019\quad (extinctions\ from\ {\it Gaia}\ DR2\ {\tt StarHorse})' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight=av50-av50_sh2019 \
      combine=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sh2019_skydiff_av.png
  
topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
    auxmap=rdbu  auxflip=true auxquant=20 auxmin=-0.5 auxmax=0.5 \
   auxvisible=true auxlabel='logg50 - logg50_{SH2019}\qquad [dex]' \
   title='Comparison\ to\ Anders+2019\quad ([M/H]\ from\ {\it Gaia}\ DR2\ {\tt StarHorse})' legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits \
      lon=l lat=b weight=met50-met50_sh2019 \
      combine=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sh2019_skydiff_met.png

# extinction prior

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false  texttype=latex fontsize=23 fontstyle=serif \
   auxmap=magma auxmin=0 auxmax=4 legend=false \
   auxvisible=true auxlabel='AV\ prior\ (median\ per\ HealPix)' \
   lon=l lat=b \
   layer_1=SkyDensity \
      in_1=/home/hpc/comas/fanders/Gaia_SH/data/SH_EDR3_results_randomset.fits \
      weight_1=AV_prior \
      combine_1=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_av_prior.png

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false  texttype=latex fontsize=23 fontstyle=serif \
   auxmap=magma auxmin=0 auxmax=4 legend=false \
   auxvisible=true auxlabel='\sigma_{AV\ prior}\ (median\ per\ HealPix)' \
   lon=l lat=b \
   layer_1=SkyDensity \
      in_1=/home/hpc/comas/fanders/Gaia_SH/data/SH_EDR3_results_randomset.fits \
      weight_1=AV_prior_error \
      combine_1=median \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_av_prior_error.png

##################

# Uncertainties vs. G

topcat -stilts plot2plane \
   xpix=595 ypix=487 \
   xlabel='G\quad [mag]' \
    ylabel='\sigma_{T{eff}}\qquad [K]' texttype=latex \
    fontsize=19 \
   xmin=10 xmax=18.5 ymin=0 ymax=600 \
   auxmap=heat auxclip=0,0.469 auxfunc=sqrt auxmin=1 \
    auxmax=371 \
   auxvisible=true auxlabel='density\qquad [arb.\ units]' \
   legend=true legpos=0.082,0.913 \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits x=phot_g_mean_mag smooth=0.2 \
   layer_1=Grid \
      y_1='0.5*(teff84-teff16)' \
      xbinsize_1=-123 ybinsize_1=-114 combine_1=count \
      leglabel_1='StarHorse2021\ (This\ work)' \
   layer_2=Quantile \
      y_2='0.5*(teff84-teff16)' \
      thick_2=7 \
      leglabel_2='StarHorse2021\ (This\ work)' \
   layer_3=Quantile \
      y_3='0.5*(teff84_SH2019-teff16_SH2019)' \
      color_3=black thick_3=5 \
      leglabel_3='StarHorse2019\ (A19)' \
   layer_4=Quantile \
      y_4=sig_Teff_Bai2019a \
      color_4=magenta thick_4=5 \
      leglabel_4=Bai+2019 \
   layer_5=Quantile \
      y_5='0.5*(teff_percentile_upper-teff_percentile_lower)' \
      color_5=cyan thick_5=5 \
      leglabel_5=Andrae+2018 \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sigteff_vs_G.png
  
topcat -stilts plot2plane \
   xpix=595 ypix=487 \
   xlabel='G\quad [mag]' ylabel='\sigma_{AV}\qquad [mag]' \
    texttype=latex fontsize=19 \
   xmin=10 xmax=18.5 ymin=0 ymax=0.5 \
   auxmap=heat auxclip=0,0.469 auxfunc=sqrt auxmin=1 \
    auxmax=520 \
   auxvisible=true auxlabel='density\qquad [arb.\ units]' \
   legend=true legpos=0.082,0.913 \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits x=phot_g_mean_mag smooth=0.2 \
   layer_1=Grid \
      y_1='0.5*(av84-av16)' \
      xbinsize_1=-123 ybinsize_1=-114 combine_1=count \
      leglabel_1='StarHorse2021\ (This\ work)' \
   layer_2=Quantile \
      y_2='0.5*(av84-av16)' \
      thick_2=7 \
      leglabel_2='StarHorse2021\ (This\ work)' \
   layer_3=Quantile \
      y_3='0.5*(av84_SH2019-av16_SH2019)' \
      color_3=black thick_3=5 \
      leglabel_3='StarHorse2019\ (A19)' \
   layer_4=Quantile \
      y_4='3.1*sig_e_bp_rp_Bai2019b' \
      color_4=magenta thick_4=5 \
      leglabel_4=Bai+2020 \
   layer_5=Quantile \
      y_5='0.5*0.89*(a_g_percentile_upper-a_g_percentile_lower)' \
      color_5=cyan thick_5=5 \
      leglabel_5=Andrae+2018 \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sigav_vs_G.png
  
topcat -stilts plot2plane \
   xpix=595 ypix=487 \
   xlabel='G\quad [mag]' ylabel='\sigma_{d}/d' \
    texttype=latex fontsize=19 \
   xmin=10 xmax=18.5 ymin=0 ymax=0.5 \
   auxmap=heat auxclip=0,0.469 auxfunc=sqrt auxmin=1 \
    auxmax=443 \
   auxvisible=true auxlabel='density\qquad [arb.\ units]' \
   legend=true legpos=0.082,0.913 \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits x=phot_g_mean_mag smooth=0.2 \
   layer_1=Grid \
      y_1='0.5*(dist84-dist16)/dist50' \
      xbinsize_1=-123 ybinsize_1=-114 combine_1=count \
      leglabel_1='StarHorse2021\ (This\ work)' \
   layer_2=Quantile \
      y_2='0.5*(dist84-dist16)/dist50' \
      thick_2=7 \
      leglabel_2='StarHorse2021\ (This\ work)' \
   layer_3=Quantile \
      y_3='0.5*(dist84_SH2019-dist16_SH2019)/dist50_SH2019' \
      color_3=black thick_3=5 \
      leglabel_3='StarHorse2019\ (A19)' \
   layer_4=Quantile \
      y_4='0.5*(r_hi_geo-r_lo_geo)/r_med_geo' \
      color_4=0099ff thick_4=5 \
      leglabel_4='Bailer\mbox{-}Jones+2021\ (geometric)' \
   layer_5=Quantile \
      y_5='0.5*(r_hi_photogeo-r_lo_photogeo)/r_med_photogeo' \
      color_5=3300ff thick_5=5 \
      leglabel_5='Bailer\mbox{-}Jones+2021\ (photo\mbox{-}geometric)' \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sigdist_vs_G.png
  
topcat -stilts plot2plane \
   xpix=595 ypix=487 \
   xlabel='G\quad [mag]' ylabel='\sigma_{\log g}\qquad [dex]' \
    texttype=latex fontsize=19 \
   xmin=10 xmax=18.5 ymin=0 ymax=0.5 \
   auxmap=heat auxclip=0,0.469 auxfunc=sqrt auxmin=1 \
    auxmax=520 \
   auxvisible=true auxlabel='density\qquad [arb.\ units]' \
   legend=true legpos=0.082,0.913 \
   in=/home/friedel/Downloads/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits x=phot_g_mean_mag smooth=0.2 \
   layer_1=Grid \
      y_1='0.5*(logg84-logg16)' \
      xbinsize_1=-123 ybinsize_1=-114 combine_1=count \
      leglabel_1='StarHorse2021\ (This\ work)' \
   layer_2=Quantile \
      y_2='0.5*(logg84-logg16)' \
      thick_2=7 \
      leglabel_2='StarHorse2021\ (This\ work)' \
   layer_3=Quantile \
      y_3='0.5*(logg84_SH2019-logg16_SH2019)' \
      color_3=black thick_3=5 \
      leglabel_3='StarHorse2019\ (A19)' \
  out=/home/friedel/Downloads/sh2021_siglogg_vs_G.png
  
topcat -stilts plot2plane \
   xpix=595 ypix=487 \
   xlabel='G\quad [mag]' ylabel='\sigma_{[M/H]}\qquad [dex]' \
    texttype=latex fontsize=19 \
   xmin=10 xmax=18.5 ymin=0 ymax=0.5 \
   auxmap=heat auxclip=0,0.469 auxfunc=sqrt auxmin=1 \
    auxmax=520 \
   auxvisible=true auxlabel='density\qquad [arb.\ units]' \
   legend=true legpos=0.082,0.913 \
   in=/home/friedel/Downloads/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits x=phot_g_mean_mag smooth=0.2 \
   layer_1=Grid \
      y_1='0.5*(met84-met16)' \
      xbinsize_1=-123 ybinsize_1=-114 combine_1=count \
      leglabel_1='StarHorse2021\ (This\ work)' \
   layer_2=Quantile \
      y_2='0.5*(met84-met16)' \
      thick_2=7 \
      leglabel_2='StarHorse2021\ (This\ work)' \
   layer_3=Quantile \
      y_3='0.5*(met84_SH2019-met16_SH2019)' \
      color_3=black thick_3=5 \
      leglabel_3='StarHorse2019\ (A19)' \
  out=/home/friedel/Downloads/sh2021_sigmet_vs_G.png
  
topcat -stilts plot2plane \
   xpix=595 ypix=487 \
   xlabel='G\quad [mag]' ylabel='\sigma_{M_{\ast}}\qquad [mag]' \
    texttype=latex fontsize=19 \
   xmin=10 xmax=18.5 ymin=0 ymax=0.5 \
   auxmap=heat auxclip=0,0.469 auxfunc=sqrt auxmin=1 \
    auxmax=443 \
   auxvisible=true auxlabel='density\qquad [arb.\ units]' \
   legend=true legpos=0.082,0.913 \
   in=/home/friedel/Downloads/SH2021_randomsample_vs_BJ21+Bai19+A18+SH19.fits x=phot_g_mean_mag smooth=0.2 \
   layer_1=Grid \
      y_1='0.5*(mass84-mass16)/mass50' \
      xbinsize_1=-123 ybinsize_1=-114 combine_1=count \
      leglabel_1='StarHorse2021\ (This\ work)' \
   layer_2=Quantile \
      y_2='0.5*(mass84-mass16)/mass50' \
      thick_2=7 \
      leglabel_2='StarHorse2021\ (This\ work)' \
   layer_3=Quantile \
      y_3='0.5*(mass84_SH2019-mass16_SH2019)/mass50_SH2019' \
      color_3=black thick_3=5 \
      leglabel_3='StarHorse2019\ (A19)' \
  out=/home/friedel/Downloads/sh2021_sigmass_vs_G.png
  

############################################

# Cantat-Gaudin catalogue comparison

topcat -stilts plot2plane \
   xpix=666 ypix=569 \
   xlog=true xflip=true yflip=true xlabel='T_{\rm eff}\quad [K]' \
    ylabel='\log g\qquad [K]' texttype=latex fontsize=18 \
   xmin=2396 xmax=29056 ymin=-1.17 ymax=5.24 \
   auxmap=rdbu  auxflip=true auxquant=20 auxmin=-0.5 auxmax=0.5 \
   auxvisible=true auxlabel='d_{SH2021}/d_{OC, CG+2020}-1' \
   legend=true legpos=0.192,0.952 \
   layer=Grid \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Cantat2020.fits \
       icmd='select proba_DR2>0.9' \
      x=teff50 y=logg50 weight='dist50/(0.001*DistPc_clus)-1' \
      xbinsize=-77 ybinsize=-66 combine=median \
      leglabel='Cantat\mbox{-}Gaudin+2020\ OC\ members\  (P_{memb}>0.9)' \
  out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_kiel_distcoloured_cg2020.png
  
topcat -stilts plot2plane \
   xpix=666 ypix=569 \
   xlog=true xflip=true yflip=true xlabel='T_{\rm eff}\quad [K]' \
    ylabel='\log g\qquad [K]' texttype=latex fontsize=18 \
   xmin=2396 xmax=29056 ymin=-1.17 ymax=5.24 \
   auxmap=rdbu auxflip=true auxquant=20 auxmin=-0.5 auxmax=0.5 \
   auxvisible=true auxlabel='AV_{SH2021}-AV_{OC, CG+2020}' \
   legend=false \
   layer=Grid \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Cantat2020.fits \
       icmd='select proba_DR2>0.9' \
      x=teff50 y=logg50 weight=av50-AVNN_clus \
      xbinsize=-77 ybinsize=-66 combine=median  \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_kiel_avcoloured_cg2020.png

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
   auxmap=rdbu auxflip=true auxmin=-0.5 auxmax=0.5 \
   auxvisible=true auxlabel='AV_{SH2021} - AV_{OC,CG2020}\qquad [mag]' \
   legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Cantat2020.fits icmd='select proba_DR2>0.9' \
      lon=l_DR2 lat=b_DR2 weight=av50-AVNN_clus \
      level=-4 combine=median  \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sky_avcoloured_cg2020.png

topcat -stilts plot2sky \
   xpix=1201 ypix=597 \
   projection=aitoff sex=false texttype=latex fontsize=23 fontstyle=serif \
   auxmap=rdbu auxflip=true auxmin=-0.5 auxmax=0.5 \
   auxvisible=true auxlabel='d_{SH2021}/d_{OC, CG+2020}-1' \
   legend=false \
   layer=SkyDensity \
      in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Cantat2020.fits icmd='select proba_DR2>0.9' \
      lon=l_DR2 lat=b_DR2 weight='dist50/(0.001*DistPc_clus)-1' \
      level=-4 combine=median  \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_sky_distcoloured_cg2020.png

####################################

# Cas A plots


topcat -stilts plot2plane \
   xpix=585 ypix=516 \
   xlabel=l ylabel=b texttype=latex fontsize=20 \
   xmin=111.204 xmax=112.205 ymin=-2.587 ymax=-1.631 \
   auxmap=inferno auxmin=1.5 auxmax=5 \
   auxvisible=true auxlabel=AV50 \
   title='Cas\ A\ region \quad (3.5\, kpc<dist50<4.5\, kpc)' \
    legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH_EDR3_results_CasA.fits \
    icmd='select "dist50>3.5 && dist50<4.5"' x=l y=b \
    thick=5 antialias=true \
   layer_1=Grid \
      weight_1=AV50 \
      xbinsize_1=.2 ybinsize_1=.2 combine_1=median \
   layer_2=Mark \
      shading_2=flat shape_2=x color_2=white \
   layer_3=Function \
      fexpr_3='sqrt(pow(5./60,2)-pow(x-111.734751,2))-02.129568 ' \
       color_3=black dash_3=3,3 \
   layer_4=Function \
      fexpr_4='-sqrt(pow(5./60,2)-pow(x-111.734751,2))-02.129568 ' \
       color_4=black dash_4=3,3 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_CasA_avmap_4kpc.png

topcat -stilts plot2plane \
   xpix=585 ypix=516 \
   xlabel=l ylabel=b texttype=latex fontsize=20 \
   xmin=111.204 xmax=112.205 ymin=-2.587 ymax=-1.631 \
   auxmap=inferno auxmin=1.5 auxmax=5 \
   auxvisible=true auxlabel=AV50 \
   title='Cas\ A\ region \quad (2.5\, kpc<dist50<3.5\, kpc)' \
    legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH_EDR3_results_CasA.fits \
    icmd='select "dist50>2.5 && dist50<3.5"' x=l y=b \
    thick=5 antialias=true \
   layer_1=Grid \
      weight_1=AV50 \
      xbinsize_1=.1 ybinsize_1=.1 combine_1=median \
   layer_2=Mark \
      shading_2=flat shape_2=x color_2=white \
   layer_3=Function \
      fexpr_3='sqrt(pow(5./60,2)-pow(x-111.734751,2))-02.129568 ' \
       color_3=black dash_3=3,3 \
   layer_4=Function \
      fexpr_4='-sqrt(pow(5./60,2)-pow(x-111.734751,2))-02.129568 ' \
       color_4=black dash_4=3,3 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_CasA_avmap_3kpc.png

topcat -stilts plot2plane \
   xpix=585 ypix=516 \
   xlabel=l ylabel=b texttype=latex fontsize=20 \
   xmin=111.204 xmax=112.205 ymin=-2.587 ymax=-1.631 \
   auxmap=inferno auxmin=1.5 auxmax=5 \
   auxvisible=true auxlabel=AV50 \
   title='Cas\ A\ region \quad (1.5\, kpc<dist50<2.5\, kpc)' \
    legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH_EDR3_results_CasA.fits \
    icmd='select "dist50>1.5 && dist50<2.5"' x=l y=b \
    thick=5 antialias=true \
   layer_1=Grid \
      weight_1=AV50 \
      xbinsize_1=.05 ybinsize_1=.05 combine_1=median \
   layer_2=Mark \
      shading_2=flat shape_2=x color_2=white \
   layer_3=Function \
      fexpr_3='sqrt(pow(5./60,2)-pow(x-111.734751,2))-02.129568 ' \
       color_3=black dash_3=3,3 \
   layer_4=Function \
      fexpr_4='-sqrt(pow(5./60,2)-pow(x-111.734751,2))-02.129568 ' \
       color_4=black dash_4=3,3 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_CasA_avmap_2kpc.png

#########################################

# GALAH

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlog=true xlabel='T_{\rm eff_{GALAH}} \qquad [K]' \
    ylabel='teff50_{SH2021}-T_{\rm eff_{GALAH}} \qquad [K]' texttype=latex \
    fontsize=24 \
   xmin=3000 xmax=8000 ymin=-2000 ymax=2000 \
   legend=true legpos=0.089,0.105 \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_GALAH_DR3.fits x=teff y=teff50-teff leglabel='GALAH+\ DR3' \
    antialias=true \
   layer_1=Mark \
      shading_1=density densemap_1=cubehelix \
   layer_2=Contour \
      color_2=black smooth_2=11 \
   layer_3=Quantile \
      smooth_3=1.02 \
   layer_4=Function \
      fexpr_4=0 color_4=black dash_4=8,4 \
   layer_5=Function \
      fexpr_5=500 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=-500 color_6=grey dash_6=3,3 \
   legseq=_1,_2,_3 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_galah_teffdiff.png

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlabel='\log g_{GALAH}' \
    ylabel='logg50_{SH2021}-\log g_{GALAH} \qquad [dex]' texttype=latex \
    fontsize=24 \
   xmin=0 xmax=5 ymin=-1 ymax=1 \
   legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_GALAH_DR3.fits x=logg y=logg50-logg leglabel='GALAH\ DR3\ stars' \
    antialias=true \
   layer_1=Mark \
      shading_1=density densemap_1=cubehelix \
   layer_2=Contour \
      color_2=black smooth_2=11 \
   layer_3=Quantile \
      smooth_3=0.1 \
   layer_4=Function \
      fexpr_4=0 color_4=black dash_4=8,4 \
   layer_5=Function \
      fexpr_5=.5 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=-.500 color_6=grey dash_6=3,3 \
   legseq=_1,_2,_3 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_galah_loggdiff.png

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlabel='(fe\_h+alpha\_fe)_{GALAH}' \
    ylabel='met50_{SH2021}-(fe\_h+alpha\_fe)_{GALAH} \qquad [dex]' texttype=latex \
    fontsize=24 \
   xmin=-2.5 xmax=1 ymin=-1 ymax=1 \
   legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_GALAH_DR3.fits x='fe_h+alpha_fe' y='met50-(fe_h+alpha_fe)' leglabel='GALAH\ DR3\ stars' \
    antialias=true \
   layer_1=Mark \
      shading_1=density densemap_1=cubehelix \
   layer_2=Contour \
      color_2=black smooth_2=11 \
   layer_3=Quantile \
      smooth_3=0.1 \
   layer_4=Function \
      fexpr_4=0 color_4=black dash_4=8,4 \
   layer_5=Function \
      fexpr_5=500 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=-500 color_6=grey dash_6=3,3 \
   legseq=_1,_2,_3 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_galah_metdiff.png

#################################

# Miglio

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlog=false xlabel='T_{\rm eff_{APOGEE\ DR14}} \qquad [K]' \
    ylabel='teff50_{SH2021}-T_{\rm eff_{APOGEE\ DR14}} \qquad [K]' texttype=latex \
    fontsize=24 size=4 \
   xmin=4400 xmax=5300 ymin=-500 ymax=500 \
   legend=true legpos=0.089,0.105 \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Miglio2021.fits \
    x=TEFF y=teff50-TEFF xerrhi=TEFF_ERR xerrlo=TEFF_ERR \
    yerrhi=teff84-teff50 \
    yerrlo=teff50-teff16 translevel=0.25 smooth=-4 \
   layer_1=Mark \
      icmd_1='select evstate==1' leglabel_1='RGB'\
      shading_1=flat color_1=blue \
   layer_2=XYError \
      icmd_2='select evstate==1' leglabel_2='RGB'\
      shading_2=translucent color_2=blue \
   layer_3=Mark \
      icmd_3='select evstate==2' leglabel_3='RC' \
      shading_3=flat \
   layer_4=XYError \
      icmd_4='select evstate==2'  leglabel_4='RC'\
      shading_4=translucent \
   layer_5=Function \
      fexpr_5=-500 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=500 color_6=grey dash_6=3,3 \
   layer_7=Function \
      fexpr_7=0 color_7=black dash_7=8,4 \
   layer_8=Quantile \
      icmd_8='select evstate==1' leglabel_8='RGB'\
      color_8=0066ff \
   layer_9=Quantile \
      icmd_9='select evstate==2'  leglabel_9='RC' \
      color_9=ff6666 \
   legseq=_1,_2,_3,_4,_8,_9 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_miglio_teffdiff.png

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlabel='M_{Miglio+2021}\qquad [M_{\odot}]' \
    ylabel='mass50_{SH2021}-M_{Miglio+2021}\qquad [M_{\odot}]' texttype=latex \
    fontsize=24 size=4 \
   xmin=0.75 xmax=2.8 ymin=-1.88 ymax=1.71 \
   legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Miglio2021.fits \
    x=mass y=mass50-mass xerrhi=mass_err84-mass \
    xerrlo=mass-mass_err18 yerrhi=mass84-mass50 \
    yerrlo=mass50-mass16 translevel=0.25 smooth=-4 \
   layer_1=Mark \
      icmd_1='select evstate==1' \
      shading_1=flat color_1=blue \
   layer_2=XYError \
      icmd_2='select evstate==1' \
      shading_2=translucent color_2=blue \
   layer_3=Mark \
      icmd_3='select evstate==2'\
      shading_3=flat \
   layer_4=XYError \
      icmd_4='select evstate==2' \
      shading_4=translucent \
   layer_5=Function \
      fexpr_5=.500 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=-.500 color_6=grey dash_6=3,3 \
   layer_7=Function \
      fexpr_7=0 color_7=black dash_7=8,4 \
   layer_8=Quantile \
      icmd_8='select evstate==1' \
      color_8=0066ff \
   layer_9=Quantile \
      icmd_9='select evstate==2' \
      color_9=ff6666 \
   legseq=_1,_2,_3,_4,_8,_9 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_miglio_massdiff.png

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlabel='\log g_{Miglio+2021}' \
    ylabel='logg50_{SH2021}-\log g_{Miglio+2021}\qquad [dex]' texttype=latex \
    fontsize=24 size=4 \
   xmin=2.2 xmax=3.4 ymin=-1 ymax=1 \
   legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Miglio2021.fits \
    x=logg_seis y=logg50-logg_seis xerrhi=0.02 \
    xerrlo=0.02 yerrhi=logg84-logg50 \
    yerrlo=logg50-logg16 translevel=0.25 smooth=-4 \
   layer_1=Mark \
      icmd_1='select evstate==1' \
      shading_1=flat color_1=blue \
   layer_2=XYError \
      icmd_2='select evstate==1' \
      shading_2=translucent color_2=blue \
   layer_3=Mark \
      icmd_3='select evstate==2'\
      shading_3=flat \
   layer_4=XYError \
      icmd_4='select evstate==2' \
      shading_4=translucent \
   layer_5=Function \
      fexpr_5=.500 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=-.500 color_6=grey dash_6=3,3 \
   layer_7=Function \
      fexpr_7=0 color_7=black dash_7=8,4 \
   layer_8=Quantile \
      icmd_8='select evstate==1' \
      color_8=0066ff \
   layer_9=Quantile \
      icmd_9='select evstate==2' \
      color_9=ff6666 \
   legseq=_1,_2,_3,_4,_8,_9 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_miglio_loggdiff.png

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlabel='[M/H]_{APOGEE\ DR14}' \
    ylabel='met50_{SH2021}-[M/H]_{APOGEE\ DR14}\qquad [dex]' texttype=latex \
    fontsize=24 size=4 \
   xmin=-1 xmax=.4 ymin=-1 ymax=1 \
   legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Miglio2021.fits \
    x='FE_H_APOGEE+ALPHA_M_APOGEE' y='met50-(FE_H_APOGEE+ALPHA_M_APOGEE)' xerrhi=0.05 \
    xerrlo=0.05 yerrhi=met84-met50 \
    yerrlo=met50-met16 translevel=0.25 smooth=-4 \
   layer_1=Mark \
      icmd_1='select evstate==1' \
      shading_1=flat color_1=blue \
   layer_2=XYError \
      icmd_2='select evstate==1' \
      shading_2=translucent color_2=blue \
   layer_3=Mark \
      icmd_3='select evstate==2'\
      shading_3=flat \
   layer_4=XYError \
      icmd_4='select evstate==2' \
      shading_4=translucent \
   layer_5=Function \
      fexpr_5=.500 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=-.500 color_6=grey dash_6=3,3 \
   layer_7=Function \
      fexpr_7=0 color_7=black dash_7=8,4 \
   layer_8=Quantile \
      icmd_8='select evstate==1' \
      color_8=0066ff \
   layer_9=Quantile \
      icmd_9='select evstate==2' \
      color_9=ff6666 \
   legseq=_1,_2,_3,_4,_8,_9 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_miglio_metdiff.png

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlabel='d_{Miglio+2021}\qquad [kpc]' \
    ylabel='dist50_{SH2021}/d_{Miglio+2021}-1' texttype=latex \
    fontsize=24 size=4 \
   xmin=0.18 xmax=4.5 ymin=-0.5 ymax=.5 xlog=true \
   legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Miglio2021.fits \
    x=dist y='dist50/dist-1' yerrhi='(dist84/dist-dist50/dist)' \
    yerrlo='(dist50/dist-dist16/dist)' xerrhi='dist_err18_1a-dist' \
    xerrlo='dist-dist_err18_1' translevel=0.25 smooth=-4 \
   layer_1=Mark \
      icmd_1='select evstate==1' \
      shading_1=flat color_1=blue \
   layer_2=XYError \
      icmd_2='select evstate==1' \
      shading_2=translucent color_2=blue \
   layer_3=Mark \
      icmd_3='select evstate==2' \
      shading_3=flat \
   layer_4=XYError \
      icmd_4='select evstate==2' \
      shading_4=translucent \
   layer_5=Function \
      fexpr_5=.500 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=-.500 color_6=grey dash_6=3,3 \
   layer_7=Function \
      fexpr_7=0 color_7=black dash_7=8,4 \
   layer_8=Quantile \
      icmd_8='select evstate==1' \
      color_8=0066ff \
   layer_9=Quantile \
      icmd_9='select evstate==2' \
      color_9=ff6666 \
   legseq=_1,_2,_3,_4,_8,_9 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_miglio_distdiff.png

topcat -stilts plot2plane \
   xpix=752 ypix=577 \
   xlabel='AV_{Miglio+2021}\qquad [mag]' \
    ylabel='AV50_{SH2021}-AV_{Miglio+2021}\qquad [mag]' texttype=latex \
    fontsize=24 size=4 \
   xmin=0. xmax=1.2 ymin=-1 ymax=1 \
   legend=false \
   in=/home/hpc/comas/fanders/Gaia_SH/data/SH2021_results_Miglio2021.fits \
    x=av y=av50-av xerrhi=av_err84-av \
    xerrlo=av-av_err18 yerrhi=av84-av50 \
    yerrlo=av50-av16 translevel=0.25 smooth=-4 \
   layer_1=Mark \
      icmd_1='select evstate==1' \
      shading_1=flat color_1=blue \
   layer_2=XYError \
      icmd_2='select evstate==1' \
      shading_2=translucent color_2=blue \
   layer_3=Mark \
      icmd_3='select evstate==2' \
      shading_3=flat \
   layer_4=XYError \
      icmd_4='select evstate==2' \
      shading_4=translucent \
   layer_5=Function \
      fexpr_5=.500 color_5=grey dash_5=3,3 \
   layer_6=Function \
      fexpr_6=-.500 color_6=grey dash_6=3,3 \
   layer_7=Function \
      fexpr_7=0 color_7=black dash_7=8,4 \
   layer_8=Quantile \
      icmd_8='select evstate==1' \
      color_8=0066ff \
   layer_9=Quantile \
      icmd_9='select evstate==2' \
      color_9=ff6666 \
   legseq=_1,_2,_3,_4,_8,_9 \
   out=/home/hpc/comas/fanders/Gaia_SH/im2021/sh2021_miglio_avdiff.png



